Minimizing the Signaling Overhead and Latency based on Users' Mobility Patterns

We demonstrate a distributed and a centralized 4G/5G compliant approach to minimize signaling and latency related to user mobility in cellular networks. This is crucial due to the densification of networks and the additional signaling introduced by the new 5G service based architecture. By exploiting standardized protocols, our solutions dynamically reorganize the association between nodes in Radio Access Network (RAN) and the core. We validated the proposed approaches using real user mobility datasets. Our results show that both our distributed and centralized solutions significantly reduce the signaling between core and RAN compared to the traditional approach based on geographical proximity. As a result, both approaches significantly reduce the average handover procedure processing time. Moreover, by relying on locally available information, the distributed approach can quickly adapt to changes in the user movement patterns as they happen.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/centralized_optimization_algorithm.tex <==
We adopt a complex systems approach to model our problem. The handover
occurrences are mapped into a functional topology \cite{Dzaferagic2016}, a graph
in which the nodes represent the base stations and the links between the nodes
indicate that a handover occurred between the connected nodes. Additionally, we
add weights to the links indicating the number of handovers that occurred
between two nodes.

Our goal is to minimize the number of inter-region handovers by grouping the
base stations that exchange more users into the same handover region. We refer
to the set of base stations as the set $V$, and the set of edges, that
represents handover occurrences, is referred to as $E$. Therefore, the
functional topology that models the handover relations of a network is referred
to as $G = (V,E)$. By modeling the handover occurrences as a weighted undirected
graph, the problem of minimizing the number of inter-region handovers becomes a
\ac{GPP}. Here we work under the assumption that the load on the base stations
are uniform and in order to get a balanced partition the number of nodes per
partition is going to be $|V|/2$.

The \ac{GPP} divides the set $V$ into two subsets $L$ and $R$ with the same
number of nodes $|V|/2$ (uniform partition), satisfying:

\begin{equation}
  \begin{array}{ll@{}ll}
    L \cap R = \emptyset\\
    L \cup R = V\\
    |L| = |R| = |V|/2,
  \end{array}
\end{equation}

so that the sum of the weights on the edges across $L$ and $R$ is minimized. We
introduce binary variables $x_i \in {0,1}$ and $y_{i,j} \in {0,1}$, so that $x_i$
takes the value 1 if the node $i$ is included in subset $L$ and the value 0
otherwise, and $y_{i,j}$ takes the value 1 if the nodes ${i,j}$ are across $L$
and $R$ and the value 0 otherwise. We also introduce variables $w_{i,j} \in
\mathbb{N}$ that represent the weights on the links between the nodes $i$ and
$j$, which are equal to the number of handovers that happened between nodes $i$
and $j$. The \ac{GPP} can now be modeled as a linear integer optimization
problem (equation (\ref{eq:optimization})).

\begin{equation}\label{eq:optimization}
\begin{array}{ll@{}ll}
\text{minimize}&\displaystyle\sum\limits_{\{i,j\}\in E} w_{i,j} \cdot y_{i,j} &\\ \\
\text{subject to}&\displaystyle\sum\limits_{i \in V}x_{i} = \frac{|V|}{2}, \\ \\
                 & x_{i} - x_{j} \leq y_{i,j}   ,   &\forall\{i,j\} \in E \\ \\
                 & x_{j} - x_{i} \leq y_{i,j}   ,   &\forall\{i,j\} \in E \\ \\
                 &x_{i} \in \{0,1\}            ,   &\forall i \in V \\ \\
                 &y_{i,j} \in \{0,1\}          ,   &\forall\{i,j\} \in E \\ \\
                 &w_{i,j} \in \mathbb{N}

\end{array}
\end{equation}

The objective is to minimize the sum of the weights on the edges across $L$ and
$R$. The first constraint ensures an equal partition ($|R| = |L| = |V|/2$). The
second and third constraint ensure that $y_{i,j} = 1$ only if nodes $i$ and $j$
are across $L$ and $R$.

Even though very powerful optimization tools exist, this approach is not the
best choice for solving this network problem. The \ac{GPP} is an NP-hard
problem, meaning that the densification of the \ac{RAN} makes this approach
infeasible. Even if we neglect the computational complexity of the problem, this
approach still assumes that the information of all the handovers is collected at
a centralized node, which involves a huge amount of signaling. The signaling
overhead of the whole network increases, and at the same time the
reconfiguration of the network is delayed due to the multiple stages in the
network optimization (collecting the handover information at the base stations,
transferring those information to a centralized node in the core network,
running the optimization software and transferring signaling messages in order
to perform the reconfiguration of the network).


% This section includes:
% \begin{enumerate}
% \item benchmarking
% \item NP-hard GPP
% \item define GPP model (mathematical definition from my notes)
% \item METIS library - we outperform this approach even though this is a well
%   known library
% \item explain the centralized approach and emphasize that the problem is
%   NP-hard - emphasize the benefits of using a distributed approach over the
%   centralized. Differences from the survey paper:
%   \begin{itemize}
%   \item centralized: 1. easy to monitor and manage; 2. high latency;
%   \item distributed: all opposite + Fog computing
%   \end{itemize}
% \item Highlight the problems of the centralized approach:
%   \begin{itemize}
%   \item signaling storm
%   \item NP-hardness
%   \item scalability
%   \item reliability
%   \item flexibility (this is related to the dynamic resource allocation)
%   \end{itemize}

% \item ADD MORE HERE BASED ON OTHER NOTES
% \end{enumerate}

==> sections/literature_review.tex <==
 Mechanism to minimize the number of \ac{SGW} relocations have been proposed in \cite{kunz2010minimizing,taleb2013gateway}. While \ac{MME} relocation is also mentioned, in both works the  focus is on the \ac{SGW}. Moreover, the implications in terms of  standards and the integration with existing or future networks are not discussed.  
% However, the centralized nature of the proposed solution would require the introduction of new protocol messages and an increase in the signaling overhead.
% Moreover, since the proposed solution relies on a distributed approach based on local information, it is able to scale with the size of the infrastructure. 
An approach specifically designed for inter-region handover optimization has been proposed in \cite{moradi2014softmow2}. However, this work relies on a new network architecture. In contrast to these previous works, our solution is designed to work within 4G and 5G networks so as to maximize technology adoption.
%In contrast, our solution exploits standardized protocols and mechanisms, which will facilitate its adoption.
In the case of femto cells, specific solutions that aim at minimizing  handover latency by reducing the signaling to and from an \ac{MME}  have been proposed  \cite{qian2014optimized, xu2011apparatus}.   Our network-wide approach is not restricted to the specific femto cell case and takes into account users' mobility when optimizing the nodes configuration. In \cite{velamati2015system, chowdhury2013dynamic}  a mechanism to re-assign \acp{BS} to \acp{MME} so as to balance the load of the \acp{MME} is proposed. Our solution, while also considering the load, re-configures the nodes based on user movements.

% Our solution is a general approach to node to x-area association, where x can be a handover region, a \ac{TA} or a set of TAs. Therefore, closely related to the question addressed by our solution is the autonomous configuration of TAs and TA Lists. Several solutions aiming at minimizing the signaling overhead caused by the periodic TA updates and paging have been developed in the research literature \cite{aqeeli2018dynamic} or patented \cite{wang2014method, singh2014tracking}. The approaches in \cite{aqeeli2018dynamic, wang2014method, singh2014tracking} are  centralized and require information that does not exist in the network (e.g. the \ac{UE} average speed, the average number of \ac{UE} per cell). Additionally, the authors do not provide implementation details in terms of data collection, and reconfiguration of the nodes. In contrast, our approach relies only on  information available in the network allowing an easy integration with the existing 4G and future 5G systems.  
% \vspace{-1.0em}
%The main contributions of this paper are:
%  \begin{itemize}
%  \item We introduce a 4G/5G compliant Network Level Mobility Management Optimization solution based on UE Mobility to minimize signaling (i.e., handover signaling, paging and tracking area updates) and handover latency by dynamically reconfiguring the association between nodes in the Radio Access Network (RAN) and nodes (e.g. Mobility Management Entity), functions (e.g. Access and Mobility Management Function) and Location Regions (e.g.Tracking Area, Registration Area, Tracking Area List) in the core network;
%  \item We make the argument that the flexible resource allocation provided by technologies like \ac{SDN} and \ac{NFV} should be paired with a flexible network organization in order to achieve dynamic up and down-scaling of network functions;
%  \end{itemize}



% This section includes:
% \begin{enumerate}
% \item white papers
% \item standards (3gpp, etsi)
% \item survey and references from the survey
% \item the reference from the survey that is the closest to the work I do
%   (SOFTMOW) - the differences are in my notes
% \item emphasize that all new approaches involve either new architectures or
%   protocols whereas our algorithm uses information that are already there based
%   on the standards
% \item I did a literature review:
%   \begin{itemize}
%   \item our algorithms perfectly aligns with the dynamic auto-scaling algorithms proposed for the SDN and NFV 
%   \item it is not just about reducing the number of handoffs, it also reduces the amount of signaling like Paging, location area updates etc. 
%   \item avoid over-provisioning of the network resources (which is the case in traditional networks)
%   \item SDN and NFV allows us to scale the control and user plane separately (our approach additionally relaxes the control plane) 
%   \item found additional motivation in terms of network flexibility, scalability and dynamic resource allocation
%   \item found a paper that has the same goal, but they used different tools which are architecture specific
%   \item Standards: the problem is still interesting even for the 5G (Even though our approach is architecture agnostic, I believe that we should go with the SDN+NFV architecture when we explain how it works because it is backwards compatible)
%   \item Companies like Nokia, Ericsson etc. are talking about the problems with
%     scalability, reliability and availability in the nextGen networks:
%     \begin{itemize}
%     \item it is always the problem with the control plane, due to the massive increase in signaling
%     \item we target a very specific part of this problem (we introduce self-organization in the RAN in order to reduce the needed amount of signaling)
%     \end{itemize}
%   \item The part that we are adding is: The network resources are flexible, therefore the nodes demanding those resources should be flexible in terms of their assignment as well.

%   \end{itemize}
%   \item ADD MORE HERE BASED ON OTHER NOTES
% \end{enumerate}
